Mitigating Malicious Attacks in Federated Learning via Confidence-aware Defense

Federated Learning (FL) is a distributed machine learning diagram that enables multiple clients to collaboratively train a global model without sharing their private local data. However, FL systems are vulnerable to attacks that are happening in malicious clients through data poisoning and model poisoning, which can deteriorate the performance of aggregated global model. Existing defense methods typically focus on mitigating specific types of poisoning and are often ineffective against unseen types of attack. These methods also assume an attack happened moderately while is not always holds true in real. Consequently, these methods can significantly fail in terms of accuracy and robustness when detecting and addressing updates from attacked malicious clients. To overcome these challenges, in this work, we propose a simple yet effective framework to detect malicious clients, namely Confidence-Aware Defense (CAD), that utilizes the confidence scores of local models as criteria to evaluate the reliability of local updates. Our key insight is that malicious attacks, regardless of attack type, will cause the model to deviate from its previous state, thus leading to increased uncertainty when making predictions. Therefore, CAD is comprehensively effective for both model poisoning and data poisoning attacks by accurately identifying and mitigating potential malicious updates, even under varying degrees of attacks and data heterogeneity. Experimental results demonstrate that our method significantly enhances the robustness of FL systems against various types of attacks across various scenarios by achieving higher model accuracy and stability.

==> checklist.tex <==
\section*{Reproducibility Checklist}

Please respond “\textbf{yes}” to each of the following questions if the relevant information is provided either in the main paper or in a technical appendix with explicit reference from the main text. If you need to provide additional explanations for any answers, please include them in a section titled “Reproducibility Checklist” at the end of the technical appendix.

\subsection*{Conceptual Clarity}
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \textbf{yes}
    \item Clearly delineates statements that are opinions, hypotheses, and speculation from objective facts and results: \textbf{yes}
    \item Provides well-marked pedagogical references for less-familiar readers to gain the necessary background to replicate the paper: \textbf{yes}
\end{itemize}

\subsection*{Theoretical Contributions (If Applicable)}
Does this paper make theoretical contributions? \textbf{yes}

If yes, please complete the following:

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally: \textbf{yes}
    \item All novel claims are stated formally (e.g., in theorem statements): \textbf{yes}
    \item Proofs of all novel claims are included: \textbf{yes}
    \item Proof sketches or intuitions are provided for complex and/or novel results: \textbf{yes}
    \item Appropriate citations to theoretical tools used are given: \textbf{yes}
    \item All theoretical claims are demonstrated empirically to hold: \textbf{yes}
    \item All experimental code used to eliminate or disprove claims is included: \textbf{yes}
\end{itemize}

\subsection*{Dataset Usage (If Applicable)}
Does this paper rely on one or more datasets? \textbf{yes}

If yes, please complete the following:

\begin{itemize}
    \item A motivation is provided for why the experiments are conducted on the selected datasets: \textbf{yes}
    \item All novel datasets introduced in this paper are included in a data appendix: \textbf{NA}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes: \textbf{NA}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations: \textbf{yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available: \textbf{yes}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying: \textbf{NA}
\end{itemize}
